Measurement of the top quark charge in pp collisions at sqrt(s) = 7 TeV with the ATLAS detector

A measurement of the top quark electric charge is carried out in the ATLAS experiment at the Large Hadron Collider using 2.05 fb-1 of data at a centre-of-mass energy of 7 TeV. In units of the elementary electric charge, the top quark charge is determined to be 0.64 +- 0.02 (stat.) +- 0.08 (syst.) from the charges of the top quark decay products in single lepton ttbar candidate events. This excludes models that propose a heavy quark of electric charge --4/3, instead of the Standard Model top quark, with a significance of more than 8 sigma.

==> t_abstract.tex <==
The ATLAS experiment potential for the study of the top quark charge at the
center-of-mass energy of 10 TeV with an estimate for 7 TeV, is reviewed in this paper.  
An approach based on the determination of the top quark decay products charges was investigated.
Using simulated samples of \ttbar events with  the \SM\
top quark decay ($\mathrm{t\rightarrow bW}$) it is shown that the ATLAS
experiment can reliably distinguish, at 5 $\sigma $ confidence level, between
the \SM\ hypothesis and the exotic one at the integrated luminosity of $\sim$
50 pb$^{-1}$ at 10 TeV and about 150 pb$^{-1}$ at 7 TeV. The expected sensitivity of the ATLAS experiment is estimated
for integrated luminosities from 10 pb$^{-1}$ to 1fb$^{-1}$ at the LHC. 

